Sequential learning and control: Targeted exploration for robust performance

We present a novel dual control strategy for uncertain linear systems based on targeted harmonic exploration and gain-scheduling with performance and excitation guarantees. In the proposed sequential approach, robust control is implemented after exploration with the main feature that the exploration is optimized with respect to the robust control performance. Specifically, we leverage recent results on finite excitation using spectral lines to determine a high probability lower bound on the resultant finite excitation of the exploration data. This provides an a priori upper bound on the remaining model uncertainty after exploration, which can further be leveraged in a gain-scheduling controller design that guarantees robust performance. This leads to a semidefinite program-based design which computes an exploration strategy with finite excitation bounds and minimal energy, and a gain-scheduled controller with probabilistic performance bounds that can be implemented after exploration. The effectiveness of our approach and its benefits over common random exploration strategies are demonstrated with an example of a system which is 'hard to learn'.

==> gain_scheduling_spectral.tex <==
%!TEX root = DualSpectral.tex
After exploration as described in Section \ref{sec:exploration}, the estimates $\hat{A}$ and $\hat{B}$ change due to the availability of new data. Since our goal is to design a stabilizing state-feedback controller that is influenced by the new estimates, the true system in \eqref{sys} is modeled as a linear parameter varying (LPV) system, where the estimates $\hat{A}_T$, $\hat{B}_T$ are measured online. The new estimates are utilized as a \textit{scheduling variable} to design a gain-scheduling controller that ensures that the closed-loop system is stable while also satisfying a quadratic performance bound.
%, e.g. $\mathcal{L}_2$ gain with high probability \cite{scherer2001lpv, veenman2014synthesis}. In particular for $x=0$ and for all signals $w\in\mathcal{L}_2$, the following inequality should hold with some $\epsilon>0$:

%\begin{align}
%\label{eq:quad_perf}
%\sum_{k=0}^{\infty}\begin{pmatrix}w_k\\z_k\end{pmatrix}^\top
%\begin{pmatrix}Q_p&S_p\\S_p^\top&R_p\end{pmatrix}
%\begin{pmatrix}w_k\\z_k\end{pmatrix}\leq -\epsilon \sum_{k=0}^{\infty}w_k^\top w_k,
%\end{align}
%where $R_p\succ 0$ is assumed.
%
%Here, we consider a generalized error that depends on the state, control input and disturbance:
%\begin{equation}\label{gz}
%z_k=Cx_k + Du_k +D_ww_k,
%\end{equation}
%where $C$, $D$ and $D_w$ are known. As a special case, the desired goal of $\mathcal{L}_2$-gain of $\gamma$ is achieved with $S_p=0$, $R_p=\frac{1}{\gamma}I$ and $Q_p=-\gamma I$ (c.f.~\cite[Prop.~3.12]{scherer2000linear}).

To account for the change in the estimates of the parameters after exploration, the system in (\ref{sys}) is rewritten as:
\begin{align}\label{gx}
x_{k+1}=&A_\mathrm{tr} x_k+B_\mathrm{tr} u_k+w_k\\\nonumber
=&\hat{A}_0x_k+\hat{B}_0u_k+(\hat{A}_T-\hat{A}_0)x_k+(\hat{B}_T-\hat{B}_0)u_k\\\nonumber
& + (A_\mathrm{tr}-\hat{A}_T)x_k +(B_\mathrm{tr}-\hat{B}_T)u_k +w_k.
\end{align}

Designing a controller for (\ref{gx}) can be written in the form of a gain-scheduling problem with an uncertain signal $w^\mathrm{u}=\Delta_\mathrm{u} \phi$ and an online measurable signal $w^\mathrm{s}=\Delta_\mathrm{s} \phi$ with the corresponding scheduling and uncertainty blocks:
\begin{equation}\label{eq:uncertainty_blocks}
\begin{split}
\Delta_\mathrm{s} & = \begin{bmatrix}
\hat{A}_T-\hat{A}_0 & \hat{B}_T-\hat{B}_0
\end{bmatrix}, \\
\Delta_\mathrm{u} & = \begin{bmatrix}
A_\mathrm{tr}-\hat{A}_T & B_\mathrm{tr}-\hat{B}_T
\end{bmatrix}.
\end{split}
\end{equation}


%\begin{equation}\label{newlpv}
%\begin{gathered}
%\begin{bmatrix}
%x_{k+1}\\z_k^s \\ z_k^u \\z_k
%\end{bmatrix}   = 
%\begin{bmatrix}
%\hat{A}_0 & I & I & I & \hat{B}_0\\
%\begin{bmatrix}
%I\\0
%\end{bmatrix} & 0 & 0 & 0 & \begin{bmatrix}
%0 \\ I
%\end{bmatrix}\\
%\begin{bmatrix}
%I\\0
%\end{bmatrix} & 0 & 0 & 0 & \begin{bmatrix}
%0 \\ I
%\end{bmatrix}\\
%C & 0 & 0 & D_w & D
%\end{bmatrix}
%\begin{bmatrix}
%x_k\\w_k^s\\w_k^u\\w_k\\u_k
%\end{bmatrix},\\
%w_k^s  = \Delta_s z_k^s,\\
%w_k^u  = \Delta_u z_k^u,
%\end{gathered}
%\end{equation}



The control input after exploration is defined as
\begin{equation}\label{eq:input}
u_k=K_\mathrm{x} x_k +K_\mathrm{s} w_k^\mathrm{s},
\end{equation}
where we use the fact that $w_k^\mathrm{s}$ is known/measurable after exploration. The controller parameters $K_\mathrm{x}$ and $K_\mathrm{s}$ are designed such that the closed-loop system is robustly stable and the specified performance criterion is met. Since the estimates $\hat{A}_T$ and $\hat{B}_T$ affect both $\Delta_\mathrm{s}$ and $\Delta_\mathrm{u}$, these blocks can be viewed as uncertain parameters, and the closed-loop uncertain system combining (\ref{gz}) and (\ref{gx}) can be written in the generalized plant form:
\begin{align}\nonumber
%\begin{gathered}
&\begin{bmatrix}
x_{k+1}\\z_k^\mathrm{s} \\ z_k^\mathrm{u} \\z_k
\end{bmatrix}  = 
\begin{bmatrix}
\hat{A}_0 + \hat{B}_0 K_\mathrm{x} & I +\hat{B}_0 K_\mathrm{s} & I & I\\
\begin{bmatrix}
I\\K_\mathrm{x}
\end{bmatrix} & \begin{bmatrix}
0 \\ K_\mathrm{s}
\end{bmatrix} & 0 & 0 \\
\begin{bmatrix}
I\\K_\mathrm{x}
\end{bmatrix} & \begin{bmatrix}
0 \\ K_\mathrm{s}
\end{bmatrix} & 0 & 0 \\ 
C+DK_\mathrm{x} & DK_\mathrm{s} & 0 & D_w
\end{bmatrix}
\begin{bmatrix}
x_k\\w_k^\mathrm{s}\\w_k^\mathrm{u}\\w_k
\end{bmatrix},\\\label{closedloop}
&\qquad\qquad\qquad\qquad\quad w_k^\mathrm{s} = \Delta_\mathrm{s} z_k^\mathrm{s},\\\nonumber
&\qquad\qquad\qquad\qquad\quad w_k^\mathrm{u} = \Delta_\mathrm{u} z_k^\mathrm{u},
%\end{gathered}
\end{align}
where $w^\mathrm{s} \rightarrow z^\mathrm{s}$ is the scheduling channel and $w^\mathrm{u} \rightarrow z^\mathrm{u}$ is the uncertainty channel.
\begin{figure}[hbtp]
\begin{center}
\includegraphics[width=0.2\textwidth]{sections/Plots/gen_plant.pdf}
\end{center}
\caption{Generalized plant view of the robust gain-scheduling problem \cite{venkatasubramanian2020robust}. }
\label{fig:GenPlant}
\end{figure}

As is apparent from Fig.~\ref{fig:GenPlant}, the closed-loop system has uncertainty and scheduling channels, affected by $\Delta_\mathrm{u}$ and $\Delta_\mathrm{s}$, respectively. The latter block $\Delta_\mathrm{s}$ is taken into account for the controller via $w_k^\mathrm{s}$ (cf.~\eqref{eq:input}), and hence plays the role of a scheduling variable. This accounts for changes in the mean of the system parameters through data gathered in the exploration phase that is available after exploration at time $T$. 

Given this formulation and suitable bounds on the blocks $\Delta_\mathrm{s}$ and $\Delta_\mathrm{u}$, the following lemma provides a matrix inequality to design a robust gain scheduling controller satisfying the performance specification defined in \eqref{eq:quad_perf}.

%\begin{lemma}
%\label{lemma:robust}
%Suppose $\Delta_\mathrm{s}\in\mathbf{\Delta}_\mathrm{s}:=\{\Delta: \Delta^\top Q_\mathrm{s} \Delta +R_\mathrm{s}\succ 0\}$, $\Delta_\mathrm{u}\in\mathbf{\Delta}_\mathrm{u}:=\{\Delta: \Delta^\top Q_\mathrm{u} \Delta  + R_\mathrm{u}\succ 0\},$  with $R_\mathrm{u},R_\mathrm{s}\succ 0$.
%%\JK{should it be strict?, I don't find the equation right now, from the set definition it should be Q positive, R negative}
%If there exists matrices $K_\mathrm{s},M,N$ and scalars $\lambda_\mathrm{s},\lambda_\mathrm{u}>0$ satisfying  the matrix inequality~\eqref{eq:LMI_gain_schedule}, then the closed loop~\eqref{closedloop} satisfies the quadratic performance bound~\eqref{eq:quad_perf} with $K_\mathrm{x}=MN^{-1}$, i.e., $u_k=MN^{-1}x_k+K_\mathrm{s} w_k^\mathrm{s}$. 
%\end{lemma}





==> gamma_bound_new.tex <==
%!TEX root = DualSpectral.tex
For causal LTI models, the $\ell_2$-gain is equal to the $H_\infty$ norm of its transfer matrix. Hence, the bound $\|V_\mathrm{tr}-\hat{V}\| \leq \gamma_\mathrm{v}$ where $\gamma_\mathrm{v}$ is the $\ell_2$-gain for the channel $u \rightarrow x$, and the bound $\|Y_\mathrm{tr}-\hat{Y}\|\leq \gamma_\mathrm{y}$ is the $\ell_2$-gain for the channel $w \rightarrow x$, of the open loop system
\begin{equation}\label{eq:open_loop}
x_{k+1}=(\hat{A}_0-A_\mathrm{tr})x_k + (\hat{B}_0-B_\mathrm{tr})u_k +w_k.
\end{equation}

The $\ell_2$-gain for the channel $u \rightarrow x$ is guaranteed to be robustly smaller than $\gamma_\mathrm{v}$ if, for $P_p=\begin{pmatrix}
-\gamma_\mathrm{v} I & 0\\0 & \frac{1}{\gamma_\mathrm{v}}I
\end{pmatrix}$, the following inequality holds for some $\epsilon>0$:
\begin{align}
\sum_{k=0}^{\infty}\begin{pmatrix}u_k\\x_k\end{pmatrix}^\top P_1 \begin{pmatrix}u_k\\x_k\end{pmatrix}\leq -\epsilon \sum_{k=0}^{\infty}u_k^\top u_k.
\end{align}

The $\ell_2$-gain for the channel $w \rightarrow x$ is guaranteed to be robustly smaller than $\gamma_\mathrm{y}$ if, for $P_2=\begin{pmatrix}
-\gamma_\mathrm{y} I & 0\\0 & \frac{1}{\gamma_\mathrm{y}}I
\end{pmatrix}$, the following inequality holds for some $\epsilon>0$:
\begin{align}
\sum_{k=0}^{\infty}\begin{pmatrix}u_k\\x_k\end{pmatrix}^\top P_p \begin{pmatrix}u_k\\x_k\end{pmatrix}\leq -\epsilon \sum_{k=0}^{\infty}u_k^\top u_k.
\end{align}


To compute $\gamma_0$, we first re-write \eqref{eq:open_loop} as
\begin{equation}\label{eq:open_loop_new}
\begin{split}
\xi_{k+1}&=\begin{bmatrix}
\hat{A}_0 & 0\\0 & A_\mathrm{tr}
\end{bmatrix} \xi_k + \begin{bmatrix}
\hat{B}_0 \\ B_\mathrm{tr}
\end{bmatrix} u_k \\
z_k & = \begin{bmatrix}
I & -I
\end{bmatrix}\xi_k
\end{split}
\end{equation}
where $\xi_k=\begin{bmatrix}x_k\\x_k\end{bmatrix}$. The prior uncertainty block is denoted as
\begin{equation}
\Delta_0=\begin{bmatrix}
A_\mathrm{tr}-\hat{A}_0 & B_\mathrm{tr}-\hat{B}_0
\end{bmatrix}.
\end{equation}
Accounting for the prior uncertainty bound and re-writing \eqref{eq:open_loop_new} in the standard form, we get
\begin{equation}\label{eq:standard_openloop}
\begin{gathered}
\begin{bmatrix}
\xi_{k+1}\\z_k^u\\z_k
\end{bmatrix}
=
\begin{bmatrix}
\begin{bmatrix}\hat{A}_0 & 0\\ 0 & \hat{A}_0 \end{bmatrix} & \begin{bmatrix}0 \\ 1 \end{bmatrix} & \begin{bmatrix} \hat{B}_0 \\ \hat{B}_0 \end{bmatrix} \\
\begin{bmatrix}
0 & I\\ 0 & 0
\end{bmatrix}& 0 & \begin{bmatrix}
0 \\ I
\end{bmatrix}  \\
\begin{bmatrix}
I & -I
\end{bmatrix} & 0 & 0
\end{bmatrix} \begin{bmatrix}
\xi_{k}\\w_k^u\\u_k
\end{bmatrix},\\
w_k^u = \Delta_0 z_k^u.
\end{gathered}
\end{equation}
Given \eqref{eq:standard_openloop}, $\gamma_0$ is a valid $H_\infty$ bound if there exists an $X \succ 0$ and a multiplier $P_p$ of the form given earlier, such that
\begin{equation}\label{eq:openloop_Hinf}
\begin{split}
\left[\begin{array}{c}
*\\ *\\ \hline
*\\ *\\ \hline
*\\ *
\end{array}\right]^\top & \left[ \begin{array}{c|c|c}
\begin{matrix}-X & 0 \\ 0 & X \end{matrix} &
\begin{matrix}0&0\\0&0\end{matrix}&
\begin{matrix}0&0\\0&0\end{matrix}\\ \hline
\begin{matrix}0&0\\0&0\end{matrix}& P_u & \begin{matrix}0&0\\0&0\end{matrix}\\ \hline
\begin{matrix}0&0\\0&0\end{matrix}&
\begin{matrix}0&0\\0&0\end{matrix}&
P_p
\end{array}\right]\\ & \times \left[\begin{array}{ccc}
I & 0 & 0\\
\begin{bmatrix}\hat{A}_0 & 0\\ 0 & \hat{A}_0 \end{bmatrix} & \begin{bmatrix}0 \\ 1 \end{bmatrix} & \begin{bmatrix} \hat{B}_0 \\ \hat{B}_0 \end{bmatrix}\\ \hline
0 & I & 0\\
\begin{bmatrix}
0 & I \\ 0 & 0
\end{bmatrix}& 0 & \begin{bmatrix}
0 \\ I
\end{bmatrix} \\ \hline
0 & 0 & I\\
\begin{bmatrix}
I & -I
\end{bmatrix} & 0 & 0
\end{array} \right]<0
\end{split}
\end{equation}
where $P_u=\begin{bmatrix}-I&0\\0&D_0^{-1}\end{bmatrix}$ and $D_0$ quantifies the uncertainty associated with $\Delta_0$ (c.f. Lemma \ref{lemma:robust} and Assumption \ref{a1}). Defining $X=N^{-1}$ and multiplying the Schur complement of  \eqref{eq:openloop_Hinf} from left and right by $\text{diag}(N,I,I)$ gives \eqref{eq:openloop_Hinf_Schur}:
\begin{footnotesize}
\begin{align}\label{eq:openloop_Hinf_Schur}
\begin{bmatrix}
\begin{array}{c|c}
\begin{bmatrix}
-N & 0 & 0\\0 & -I & 0\\0 & 0 & -\gamma_0 I
\end{bmatrix} & \star \\ \hline
\begin{bmatrix}
\begin{bmatrix}\hat{A}_0 N & 0\\ 0 & \hat{A}_0 N \end{bmatrix} & \begin{bmatrix} \hat{B}_0 \\ \hat{B}_0 \end{bmatrix} & \begin{bmatrix}0 \\ 1 \end{bmatrix}\\
\begin{bmatrix}0 & N \\ 0 & 0\end{bmatrix} & \begin{bmatrix}0 \\ 1 \end{bmatrix} & 0 \\
\begin{bmatrix}I & -I\end{bmatrix} & 0 & 0
\end{bmatrix} & \begin{bmatrix}
-N & 0 & 0\\0 & -D_0 & 0\\0 & 0 & -\gamma_0 I
\end{bmatrix}
\end{array}
\end{bmatrix} \prec 0
\end{align}
\end{footnotesize}



==> opnorm_bound.tex <==
\remove{\begin{definition}{(Sub-Gaussian norm \cite[Definition 2.5.6]{vershynin2018high})}\label{def:subg_norm} The sub-Gaussian norm of a sub-Gaussian random variable $X$, denoted as $\|X\|_{\psi_2}$, is defined as
\begin{equation}
\|X\|_{\psi_2}=\inf \left\{ t>0 : E\left(\textnormal{exp}(X^2/t^2)\right)\leq 2\right\}
\end{equation}
\end{definition}
\begin{remark}\label{rem:subg_norm_gauss} If $X \sim \mathcal{N}(0,\sigma^2)$, then X is sub-Gaussian with $\|X\|_{\psi_2} \leq C_s \sigma$ where $C_s$ is an absolute constant.
\end{remark}
Given the definition of the sub-Gaussian norm, the following theorem provides an upper-bound on the operator norm of a random matrix whose entries are sub-Gaussian.
\begin{theorem}{\cite[Theorem 4.4.5]{vershynin2018high}}\label{lem:w_norm_bound} Let $W$ be a $m \times n$ random matrix whose entries $W_{ij}$ are independent, zero mean, sub-Gaussian random variables. Then, for any $t>0$ we have
\begin{equation}\label{eq:w_normbound}
\|W\| \leq C_s L(\sqrt{m}+\sqrt{n}+t)
\end{equation}
with probability at least $1-2\,\textnormal{exp}(-t^2)$. Here $C_s$ is some positive absolute constant and $L=\max_{i,j} \|W_{ij}\|_{\psi_2}$.
\end{theorem}
\begin{proof}
This proof utilizes the $\varepsilon$-net argument to control the operator norm. Choose $\varepsilon=1/4$. The sizes of $\varepsilon$-nets $\mathcal{N}$ of $\mathcal{S}^{n-1}$ and $\mathcal{M}$ of $\mathcal{S}^{m-1}$ are $|\mathcal{N}| \leq 9^n$ and $|\mathcal{M}| \leq 9^m$ \cite[Corrollary 4.2.13]{vershynin2018high}. For the chosen value of $\varepsilon$, the operator norm can be bounded using $\varepsilon$-nets as
\begin{equation}
\|W\| \leq 2 \max_{x\in \mathcal{N},y \in \mathcal{M}} \left< Wx,y \right>.
\end{equation}
For a fixed $x \in \mathcal{N}$ and $y \in \mathcal{M}$, the quadratic form $\left< Wx,y \right>$ is a sum of independent, sub-Gaussian random variables and $\|\left< Wx,y \right>\|^2_{\psi_2}=C_s L^2$. This can be restated as the tail bound \cite[(2.14)]{vershynin2018high}, for $l \geq 0$ as
\begin{equation}
\mathbb{P}\{\left<Wx,y\right> \geq l \} \leq 2\, \textnormal{exp}(-c_s l^2/L^2).
\end{equation}
Furthermore, unfixing $x$ and $y$ using a union bound yields
\begin{equation}
\mathbb{P}\left\{ \max_{x \in \mathcal{N},y \in \mathcal{M}} \left< Wx,y \right> \geq l \right\} \leq \sum_{x \in \mathcal{N},y \in \mathcal{M}} \mathbb{P} \left\{ \left<Wx,y \right> \geq l \right\}.
\end{equation}
Given the sizes of $\mathcal{N}$ and $\mathcal{M}$, and by the definition of the operator norm, the probability stated above is bounded by
\begin{equation}\label{eq:prob_w}
\mathbb{P}\left\{ \|W\| \geq 2l \right\} \leq 9^{n+m} \cdot 2 \, \textnormal{exp}(-c_s l^2/L^2).
\end{equation}
Choose $l=C_s L(\sqrt{n}+\sqrt{m}+t)$ and $C_s$ sufficiently large such that the exponent is large enough. Then,
\begin{equation}
\mathbb{P}\left\{ \|W\| \geq 2l \right\} \leq 2\, \textnormal{exp}(-t^2).\qedhere
\end{equation}\qedhere
\end{proof}
\begin{corollary}{(Expected norm)}\label{cor:exp_norm} Let $W$ be a $m \times n$ random matrix whose entries $W_{ij}$ are independent, zero mean, sub-Gaussian random variables. Then,
\begin{align}
\mathbb{E}\left( \|W\| \right) \leq C_s L (\sqrt{m}+\sqrt{n})
\end{align}
where $C_s$ is some positive absolute constant and $L=\max_{i,j} \|W_{ij}\|_{\psi_2}$.
\end{corollary}}
%Subsumed within the above lemma is the following probabilistic bound. If $W \sim \mathcal{N}(0,\sigma_{\bar{w}}^2)$, then $L \leq C_s \sigma_{\overline{w}}$ and from \eqref{eq:prob_w}, we have
%\begin{equation}
%\mathbb{P}\left\{ ||W|| \geq 2l \right\} \leq 9^{n+m} \cdot 2 \, \textnormal{exp}(-c_s l^2/C_s^2 \sigma_{\bar{w}}^2)
%\end{equation}

